Measurement of the Longitudinal Proton Structure Function at HERA

The reduced cross sections for ep deep inelastic scattering have been measured with the ZEUS detector at HERA at three different centre-of-mass energies, 318, 251 and 225 GeV. From the cross sections, measured double differentially in Bjorken x and the virtuality, Q^2, the proton structure functions FL and F2 have been extracted in the region 5*10^-4 < x <0.007 and 20 < Q^2 < 130 GeV^2.

==> LaTeX/examples/conf/zconf-cit.tex <==
%==============================================================================
%	Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
%	-> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
%	-> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
%	-> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}


==> LaTeX/examples/conf/zconf-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{<comma-separated list of bib files>}}
}
\vfill\eject


==> LaTeX/examples/conf/zconf-tit.tex <==
\prepnum{DESY--11--NNN}

\title{
Search for a Better Life\\
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering\\
at HERA
}                                                       
                    
\author{ZEUS Collaboration}
\draftversion{0.1}
\date{27.\ May 2011}

\confname{XXX$^{\rm th}$ International Conference on High Energy Physics}
\confplacedate{Osaka, Japan, July 27 -- August 2, 2000}
\confsession{Plenary Session: M\\Parallel Session: K}
\confabsnum{9999}

\abstract{
In a search for a better life beyond the Standard Model, various hypotheses have
been tested using the high--$Q^2$, deep inelastic neutral--current $e^+p$
scattering data collected with the ZEUS detector at HERA.  The data correspond
to an integrated luminosity of $47.7\pbi$ of $e^+p$ interactions at $300\gev$
center-of-mass energy. No significant evidence for holidays has been found.
Lower limits at the $95\%$ confidence level are set on the average monthly
working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/conf/zconf-txt.tex <==
\pagenumbering{arabic} 
\pagestyle{plain}
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.
\vfill\eject


==> LaTeX/examples/draft/zdraft-fig.tex <==
%-------------------------------------------------------------------------------
%       Results
%-------------------------------------------------------------------------------
\begin{figure}[p]
\vfill
\begin{center}
\framebox[13.cm]{\rule{0.pt}{10.cm}}
\end{center}
\caption{
Life beyond the Standard Model.}
\label{fig-contfey}
\vfill
\end{figure}


==> LaTeX/examples/draft/zdraft-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{<comma-separated list of bib files>}}
}
\vfill\eject


==> LaTeX/examples/draft/zdraft-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> LaTeX/examples/draft/zdraft-tit.tex <==
\title{
Search for a Better Life\\
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering\\
at HERA
}                                                       
                    
\author{ZEUS Collaboration}
\draftversion{0.1}
\date{27.\ May 2011}

\abstract{
In a search for a better life beyond the Standard Model, various hypotheses have
been tested using the high-$Q^2$, deep inelastic neutral current $e^+p$
scattering data collected with the ZEUS detector at HERA.  The data correspond
to an integrated luminosity of $47.7\pbi$ of $e^+p$ interactions at $300\gev$
center-of-mass energy. No significant evidence for holidays has been found.
Lower limits at the $95\%$ confidence level are set on the average monthly
working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/draft/zdraft-txt.tex <==
\pagenumbering{arabic} 
\pagestyle{plain}
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc\ZcoosysfnBeta

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty for your sample as argument
% ----------------------------------------------------------------------------
\Zlumidesc{2.6~\%}

\vfill\eject


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.c
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\vfill\eject


==> LaTeX/examples/note/znote-cit.tex <==
%==============================================================================
%	Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
%	-> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
%	-> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
%	-> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}


==> LaTeX/examples/note/znote-fig.tex <==
%-------------------------------------------------------------------------------
%       Results
%-------------------------------------------------------------------------------
\begin{figure}[p]
\vfill
\begin{center}
\framebox[13.cm]{\rule{0.pt}{10.cm}}
\end{center}
\caption{
Life beyond the Standard Model.}
\label{fig-contfey}
\vfill
\end{figure}


==> LaTeX/examples/note/znote-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{<comma-separated list of bib files>}}
}
\vfill\eject


==> LaTeX/examples/note/znote-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> LaTeX/examples/note/znote-tit.tex <==
\prepnum{ZEUS--11--NNN}

\title{
Calibration of the Mood of the Operators\\
in the ZEUS running 2006/2007
}                                                    
                    
\author{Your name\\
        {\small\it your email}\\[3.mm]
        Your institution\\
        {\it address}\\
}
\date{27.\ May 2011}

\abstract{
In previous years, strong dependences of data taking efficiencies and 
physics results on the mood of the ZEUS shift crew have been observed.
We report on an attempt to automatically monitor and adjust the 
relevant parameters by supplying moderate doses of beer. It can be shown 
that this approach stabilizes the situation. However, remaining dependences,
in particular on the moon phase, are still to be corrected for.
}

\makezeustitle


==> LaTeX/examples/note/znote-txt.tex <==
\pagenumbering{arabic} 
\pagestyle{plain}
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots At some
place you might in particular like to introduce the CTD \citeCTD, the
MVD \citeMVD and the ZEUS calorimeter \citeCAL.
\vfill\eject


==> LaTeX/examples/other/zother-cit.tex <==
%==============================================================================
%	Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
%	-> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
%	-> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
%	-> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}


==> LaTeX/examples/other/zother-fig.tex <==
%-------------------------------------------------------------------------------
%       Results
%-------------------------------------------------------------------------------
\begin{figure}[p]
\vfill
\begin{center}
\framebox[13.cm]{\rule{0.pt}{10.cm}}
\end{center}
\caption{
Life beyond the Standard Model.}
\label{fig-contfey}
\vfill
\end{figure}


==> LaTeX/examples/other/zother-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
%
%  If you (have to) use a different bibliography style file than
%  l4z_default.bst (or one of its clones derived from zeusbtxbst.bdc),
%  you will have to apply several adjustments to it:
%  - Add the fields "checked", "eprint", "replaces" and "replacedby",
%    "report", "submitdate" and "www" to the ENTRY section.
%  - Add a appropriate definitions for entry types "Preprint" and
%    "Thesis".
%
%  You will probably decide that it is horribly complicated to get 
%  this working.
%  I offer support for two types of possible solutions:
%  (i)  try to adhere to the required standards by choosing the 
%       appropriate flags in zeusbtxbst.bdc and adapting the 
%       resulting bst file as necessary
%  (ii) take the bst file provided by the editor or publishing
%       institution and adapt it to the data fields and conventions
%       in the LaTeX4zeus bibligraphy database.
%
%  I cannot promise that either of both possibilities works, but 
%  in general there should be a solution which allows to use the 
%  LaTeX4zeus bibligraphy database. Please contact me (Uli Katz,
%  katz@physik.uni-bonn.de) for further support.
%
%                                 Good luck! Uli
%
%
%  Please report technical problems using the LaTeX4zeus message form:
%  http://www-zeus.desy.de/ZEUS_ONLY/LaTeX4zeus/WWW/php/l4z_message.php3
%
\bibliographystyle{./BiBTeX/bst/l4z_default}
{\raggedright
\bibliography{<comma-separated list of bib files>}}
}
\vfill\eject


==> LaTeX/examples/other/zother-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> LaTeX/examples/other/zother-tit.tex <==
%
%  Title page and abstract.
%  ------------------------
%  Note that the abstract is not included in the standard title page
%  of article.cls (and therefore appears on a separate page). Other
%  class files may define additional or different elements of the title
%  page.
%

\title{
A Scientific Report\\
Typeset in the \LaTeXZ Environment\\
Without Using \texttt{zeus{\usc}paper.cls}
}                                                       
                    
\author{Your name\\
        {\small\it your email}\\[3.mm]
        Your institution\\
        {\it address}\\
}
\date{27.\ May 2011}

\maketitle

\noindent{\bf Abstract:}
The \LaTeXZ environment provides access to a large bibliography
data base and a set of utility macros which can be used also outside
the framework set up in the \LaTeX{} class file \texttt{zeus{\usc}paper.cls}.
This report may serve as an example.



==> LaTeX/examples/other/zother-txt.tex <==
\pagenumbering{arabic} 
\pagestyle{plain}
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your text and futher sections and subsections \dots

At some place you might in particular like to introduce the CTD
\citeCTD, the MVD \citeMVD and the ZEUS calorimeter \citeCAL. If not,
these references may serve as examples for the use of definitions in
\texttt{zother-cit.tex}.

\vfill\eject


==> LaTeX/examples/prep/zprep-aut.tex <==
%=================================================================== 
%
%  This file will be replaced with the "official" author
%  list which is created for each ZEUS paper individually.
%
%===================================================================== 
{
\pagenumbering{Roman} 

\begin{center} 
{\Large  The ZOOPS Collaboration}
\end{center}

{\raggedright
  F.~Author$^{1}$,
  A.~Nother,
  X.~Whoever\\
 {\it Absolutely Non-Existing Institute of Nothing, Nowhere, Country}~$^{a}$ 
}

\par\filbreak
\begin{supertabular}[h]{rp{14cm}}
$^{\ 1}$ & now visiting a scientist next door\\ 
\end{supertabular}

\begin{tabular}[h]{rp{14cm}}
$^{a}$ &  supported by the National Council of Nonsense (NCNS)\\ 
\end{tabular} 
}

\clearpage


==> LaTeX/examples/prep/zprep-cit.tex <==
%==============================================================================
%	Some definitions of citations
%==============================================================================
%------------------------------------------------------------------------------
%	-> CTD
%------------------------------------------------------------------------------
\def\citeCTD{{\cite{%
nim:a279:290,*npps:b32:181,*nim:a338:254%
}}\xspace}
%------------------------------------------------------------------------------
%	-> MVD
%------------------------------------------------------------------------------
\def\citeMVD{{\cite{%
nim:a581:656%
}}\xspace}
%------------------------------------------------------------------------------
%	-> CAL
%------------------------------------------------------------------------------
\def\citeCAL{{\cite{%
nim:a309:77,*nim:a309:101,*nim:a321:356,*nim:a336:23%
}}\xspace}
%------------------------------------------------------------------------------
%	-> BAC
%------------------------------------------------------------------------------
\def\citeBAC{{\cite{%
nim:a300:480%
}}\xspace}
%------------------------------------------------------------------------------
%	-> LUMI
%------------------------------------------------------------------------------
\def\citePCAL{{\cite{%
desy-92-066,*zfp:c63:391,*acpp:b32:2025%
}}\xspace}
\def\citeSPECTRO{{\cite{%
physics-0512153%
}}\xspace}



==> LaTeX/examples/prep/zprep-fig.tex <==
%-------------------------------------------------------------------------------
%       Results
%-------------------------------------------------------------------------------
\begin{figure}[p]
\vfill
\begin{center}
\framebox[13.cm]{\rule{0.pt}{10.cm}}
\end{center}
\caption{
Life beyond the Standard Model.}
\label{fig-contfey}
\vfill
\end{figure}


==> LaTeX/examples/prep/zprep-ref.tex <==
{
\def\bibname{\Large\bf References}
\def\refname{\Large\bf References}
\pagestyle{plain}
\ifzeusbst
  \bibliographystyle{./BiBTeX/bst/l4z_default}
\fi
\ifzdrftbst
  \bibliographystyle{./BiBTeX/bst/l4z_draft}
\fi
\ifzbstepj
  \bibliographystyle{./BiBTeX/bst/l4z_epj}
\fi
\ifzbstnp
  \bibliographystyle{./BiBTeX/bst/l4z_np}
\fi
\ifzbstpl
  \bibliographystyle{./BiBTeX/bst/l4z_pl}
\fi
{\raggedright
\bibliography{<comma-separated list of bib files>}}
}
\vfill\eject


==> LaTeX/examples/prep/zprep-tab.tex <==
%-------------------------------------------------------------------------------
%       An example table
%-------------------------------------------------------------------------------
\begin{table}[p]
\begin{center}
\begin{tabular}{||c|rrrr|rrrr||}
\hline
Label & $\eta^u_{LL}$ & $\eta^u_{LR}$ & $\eta^u_{RL}$ & $\eta^u_{RR}$ & 
        $\eta^d_{LL}$ & $\eta^d_{LR}$ & $\eta^d_{RL}$ & $\eta^d_{RR}$ \\ 
\hline\hline
VV&  $+1$&$+1$&$+1$&$+1$&
     $+1$&$+1$&$+1$&$+1$ \\
AA&  $+1$&$-1$&$-1$&$+1$&
     $+1$&$-1$&$-1$&$+1$ \\
VA&  $+1$&$-1$&$+1$&$-1$&
     $+1$&$-1$&$+1$&$-1$ \\
X1&  $+1$&$-1$&$ 0$&$ 0$&
     $+1$&$-1$&$ 0$&$ 0$ \\
X2&  $+1$&$ 0$&$+1$&$ 0$&
     $+1$&$ 0$&$+1$&$ 0$ \\
X3&  $+1$&$ 0$&$ 0$&$+1$&
     $+1$&$ 0$&$ 0$&$+1$ \\
X4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$+1$&$+1$&$ 0$ \\
X5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$+1$&$ 0$&$+1$ \\
X6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$+1$&$-1$ \\
U1&  $+1$&$-1$&$ 0$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U2&  $+1$&$ 0$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U3&  $+1$&$ 0$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U4&  $ 0$&$+1$&$+1$&$ 0$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U5&  $ 0$&$+1$&$ 0$&$+1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
U6&  $ 0$&$ 0$&$+1$&$-1$&
     $ 0$&$ 0$&$ 0$&$ 0$ \\
\hline
\end{tabular}
\caption{The 30 scenarios for a better life considered in this paper.
         Each row of this table corresponds to two different scenarios for
         overall interference signs $\epsilon=+1$ and $\epsilon=-1$, 
         respectively.}
  \label{tab-models}
\end{center}
\end{table}


==> LaTeX/examples/prep/zprep-tit.tex <==
\prepnum{DESY--11--NNN}

\title{
Search for a Better Life\\
in Deep Inelastic $\mathbf{e^+p\to e^+X}$ Scattering\\
at HERA
}                                                       
                    
\author{ZEUS Collaboration}
\date{27.\ May 2011}

\abstract{
In a search for a better life beyond the Standard Model, various hypotheses have
been tested using the high-$Q^2$, deep inelastic neutral current $e^+p$
scattering data collected with the ZEUS detector at HERA.  The data correspond
to an integrated luminosity of $47.7\pbi$ of $e^+p$ interactions at $300\gev$
center-of-mass energy. No significant evidence for holidays has been found.
Lower limits at the $95\%$ confidence level are set on the average monthly
working time of a physicist.
}

\makezeustitle


==> LaTeX/examples/prep/zprep-txt.tex <==
\pagenumbering{arabic} 
\pagestyle{plain}
% ----------------------------------------------------------------------------
%       Introduction
% ----------------------------------------------------------------------------
\section{Introduction}
\label{sec-int}

Here comes your introductory text.

% ----------------------------------------------------------------------------
%       Experimental set-up
% ----------------------------------------------------------------------------
\section{Experimental set-up}
\label{sec-exp}

Here you might want to describe your data samples and the detctor. In
particular, you may use some of the text fragments provided as \LaTeXZ
macros.

% ----------------------------------------------------------------------------
%       General detector blabla
% ----------------------------------------------------------------------------
\Zdetdesc

% ----------------------------------------------------------------------------
%       CTD+MVD description, footnote on coordinate system is the argument
% ----------------------------------------------------------------------------
\Zctdmvddesc\ZcoosysfnBeta

% ----------------------------------------------------------------------------
%       CAL description straight and simple
% ----------------------------------------------------------------------------
\Zcaldesc

% ----------------------------------------------------------------------------
%       Muon system description. You may want it or not. No references for it
% ----------------------------------------------------------------------------
\Zmuondesc

% ----------------------------------------------------------------------------
%       BAC description complete with reference
% ----------------------------------------------------------------------------
\Zbacdesc

% ----------------------------------------------------------------------------
%       LUMI, give actual luminosity uncertainty for your sample as argument
% ----------------------------------------------------------------------------
\Zlumidesc{2.6~\%}

\vfill\eject


% ----------------------------------------------------------------------------
%       Mandatory acknowledgements. You may add your buddies to it.
% ----------------------------------------------------------------------------
\section*{Acknowledgements}
\label{sec-ack}

\Zacknowledge

\vfill\eject


==> LaTeX/examples/talk/ztalk-fmt.tex <==
%------------------------------------------------------------------------------
%       interline spacing, paragraph indention etc.
%------------------------------------------------------------------------------
\renewcommand{\baselinestretch}{1.0}
\renewcommand{\arraystretch}{1.1}
\parindent       0.0pt
\parskip         3.5pt
\overfullrule    0.0pt
%------------------------------------------------------------------------------
%       item spacings
%------------------------------------------------------------------------------
\itemsep    0.2ex plus 0.1ex minus 0.15ex
\topsep     0.2ex plus 0.1ex minus 0.15ex
\partopsep  0.2ex plus 0.1ex minus 0.1ex
\setlength\leftmargini   {1.6em}
\setlength\leftmarginii  {1.2em}
\setlength\leftmarginiii {1.0em}
\setlength\leftmarginiv  {0.8em}
%------------------------------------------------------------------------------
%       define colored bullet with distance for pseudo-itemize environment
%------------------------------------------------------------------------------
\def\cbullet#1{{#1\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern1.em}
\def\cbull#1#2{{#1\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern#2}
\def\carrow#1{{#1$\mbs{\to}$}\kern0.55em}
\def\cminus#1{{\bf#1--}\kern0.8em}
\def\cmin#1#2{{\bf#1--}\kern#2}
\def\cplus#1{{#1$\mbs{+}$}\kern0.8em}
\def\cplu#1#2{{#1$\mbs{+}$}\kern#2}
\def\cequal#1{{#1$\mbs{=}$}\kern0.7em}
\def\csurd#1{{#1$\mbs{\surd}$}\kern1.em}
\def\csur#1#2{{#1$\mbs{\surd}$}\kern#2}
\def\pbullet{\phantom{{\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern1.em}}
\def\pbull#1{\phantom{{\raisebox{0.3ex}{$\mbs{\bullet}$}}\kern#1}}
\def\parrow{\phantom{{$\mbs{\to}$}\kern0.55em} }
\def\pminus{\phantom{{\bf--}\kern0.8em} }
\def\pequal{\phantom{{$\mbs{=}$}\kern0.7em} }
\def\psurd{\phantom{{$\mbs{\surd}$}\kern1.em} }
\def\psur#1{\phantom{{$\mbs{\surd}$}\kern#1} }
%------------------------------------------------------------------------------
%       "tight item" environment
%------------------------------------------------------------------------------
\newenvironment{tightitemize}[2]
 {\begin{list}{$\bullet$}%
  {\setlength{\leftmargin}{\leftmargini}%
   \setlength{\topsep}{#1}%
   \setlength{\itemsep}{#2}%
  }%
 }%
 {\end{list}}
%------------------------------------------------------------------------------
%       Define mathbfs
%       --------------
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbfs}{OT1}{lcmss}{bx}{sl}
%\DeclareMathAlphabet{\mathbfs}{OT1}{cmr}{bx}{sl}
\def\mbs{\mathbfs}
%------------------------------------------------------------------------------
%       boxpage decoration
%       ------------------
%------------------------------------------------------------------------------
\newcounter{chap}
\newcounter{chapslide}
\setcounter{chapslide}{0}
\renewcommand{\footerleft}{U.~Katz}
\renewcommand{\footerright}{\thechap.\thechapslide}
\renewcommand{\footercenter}{\LaTeXZ}
\renewcommand{\bpdtcolor}{money}
\renewcommand{\bpdtype}{B}
\renewcommand{\boxpagedecoration}{%
  \strut\kern-1.7cm
  \begin{turn}{90}
    \begin{minipage}{\textheight}
      \begin{center}
        \color{darkred}
        {\tiny{\usefont{OT1}{cmr}{m}{sc}
               ZEUS Collaboration Meeting, 
               DESY, 23.--27.~Oct.~2000\stru{0.pt}{4.6mm}}}
      \end{center}
    \end{minipage}%
  \end{turn}    
  \begin{minipage}[t]{\textwidth}
    \stepcounter{chapslide}
    \color{\bpdtcolor}\rule[\footerruledist]{\textwidth}{\footerrulewidth}
    \tiny\footerleft\hfill\footercenter\hfill\footerright
  \end{minipage}%
}


==> LaTeX/examples/talk/ztalk-tit.tex <==
%-------------------------------------------------------------------------------
%       Title page
%-------------------------------------------------------------------------------
{
\begin{boxpage}[e]
%%
%%  title box
%%
{
\putboxparloc{}{1.9pt}{purple}{yellow}{purple}
\putbox{f}{ct}{t}{c}{0}{s}{0}{
  \begin{center}
    \bf\Large
    \stru{2.2ex}{0.ex}
    \LaTeXZ:\kern3.cm\\
    A \LaTeX\ Environment\kern3.cm\\[-3.mm]
    for ZEUS\kern3.cm
    \stru{0.ex}{1.5ex}
  \end{center}}%
}
%%
%%  the LaTeX lion
%%
\putbox{p}{rt}{c}{-20}{20}{350}{380}{figure=plots/lion_yellow.eps,clip=}
%%
%%  name, institute
%%
{
\putboxcolloc{blue}{}{cyan}
\putbox{b}{ct}{t}{c}{700}{s}{0}{
  \begin{center}
     Uli Katz,\\
     University of Bonn
  \end{center}}%
}
%%
%%  the ZEUS logo
%%
\putbox{p}{lt}{c}{80}{1000}{500}{500}{figure=plots/zeus_logo.eps,clip=}
%%
%%  add occasion, date
%%
{
\putboxcolloc{red}{lightyellow}{darkcyan}
\putbox{B}{rt}{c}{-0}{1000}{1070}{400}{
  \begin{center}
     \vfill
     {\large
     Collaboration Meeting}
     \vfill
     DESY, 23-27.~Oct.~2000
     \vfill
  \end{center}}%
}
%%
%%  table of contents
%%
{
\putboxparloc{4.mm}{}{green}{lightestcyan}{black}
\putbox{f}{cb}{c}{c}{-150}{1400}{0}{
    \cbull{\red}{0.7em} {\darkblue Objectives}\\[0.5mm]
    \cbull{\red}{0.7em} {\darkblue Elements}\\[0.5mm]
    \cbull{\red}{0.7em} {\darkblue The bibliography data base}\\[-1.5mm]
           \pbull{1.7em}{\darkgreen\small User interface}\\[-1.5mm]
           \pbull{1.7em}{\darkgreen\small Administration and quality checking}\\
    \cbull{\red}{0.7em} {\darkblue Status and release}
}}
%%
\end{boxpage}
}


==> LaTeX/examples/talk/ztalk-txt.tex <==
\setcounter{chap}{1}
%-------------------------------------------------------------------------------
%       Objectives
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Objectives of \LaTeXZ
  \end{center}}
}
%%
%%  List of main goals of LaTeX4zeus
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{350}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\large\magenta Support common ZEUS 
                                         paper style}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Provides well-defined appearence\\[-2.2mm]
                       \>\>(title page layout, fonts, \dots)\\
                       \>\cmin{\green}{-.5em}
                         \>Implementation of rules and conventions\\[-2.2mm]
                       \>\>in {\it The Guide for Writing ZEUS Papers}\\[7.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta Provide user-friendly}\\[-1.mm]
                       \>{\large\magenta \LaTeX\ environment}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Collection of useful \LaTeX\ macros\\
                       \>\cmin{\green}{-.5em}
                         \>Ready-to-use setup for ZEUS drafts,\\[-2.2mm]
                       \>\>preprints, notes, coference contributions\\
                       \>\cmin{\green}{-.5em}
                         \>Easy installation\\
                       \>\cmin{\green}{-.5em}
                         \>Detailed WWW documentation\\[7.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta BiBTeX data base}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Collects all references used by ZEUS\\[-2.2mm]
                       \>\>documents in one central data base.\\
                       \>\cmin{\green}{-.5em}
                         \>High quality standard (new entries\\[-2.2mm]
                       \>\>are checked by scientific editor)\\
                       \>\cmin{\green}{-.5em}
                         \>WWW interface for searching\\[-2.2mm]
                       \>\>and adding entries\\
                       \>\cmin{\green}{-.5em}
                         \>{\darkred Success depends on your 
                                     contributions!}
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Elements
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Elements of \LaTeXZ
  \end{center}}
}
%%
%%  List of main elements of LaTeX4zeus
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{270}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\large\magenta Documentation}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>{\green 
                    \texttt{http://giroz.desy.de/ZEUS{\usc}ONLY/LaTeX4zeus}}\\
                       \>\cmin{\green}{-.5em}
                         \>Installation, usage, development \dots\\
                       \>\cmin{\green}{-.5em}
                         \>Message interface\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta Installation mechanism}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>All relevant files in one gzip'ed tar file\\[-2.2mm]
                       \>\>$\Rightarrow$ download, unpack and execute\\[-2.2mm]
                       \>\>\phantom{$\Rightarrow$ }installation script\\
                       \>\cmin{\green}{-.5em}
                         \>Start working ...\\
                       \>\cmin{\green}{-.5em}
                         \>Easy migration for existing projects.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta \LaTeX\ macros}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Provide all the nice handy utilities\\[-2.2mm]
                       \>\>you always (never?) wanted to have.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta BiBTeX data base}\\[2.mm]
                       \>\cmin{\green}{-.5em}
                         \>Just select your references and use them.\\
                       \>\cmin{\green}{-.5em}
                         \>Provide missing references\\[-2.2mm]
                       \>\>using WWW interface.\\
                       \>\cmin{\green}{-.5em}
                         \>Checking, formatting etc.\ is done for you.\\[5.mm]
  \ \cbull{\red}{-.5em}\>{\large\magenta An advanced class package for slides}
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Message form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Message form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{400}{1800}{0}{figure=plots/l4z_message.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1900}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Messages are stored in WWW-accessible file\\[2.mm]
  \ \cbull{\red}{-.5em}\>Scientific editor and/or \LaTeXZ\\
                       \>developper will react a.s.a.p.
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Bibliography search form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography search form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{400}{1800}{0}{figure=plots/l4z_search1.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1750}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>You can request a logical {\it and} or {\it or}\\
                       \>of up to 5 search conditions.\\[2.mm]
  \ \cbull{\red}{-.5em}\>Note that search is done in BiBTeX files\\
                       \>containing LaTeX syntax.\\[2.mm]
  \ \cbull{\red}{-.5em}\>Online help available
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Bibliography search results
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography search results
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{550}{1800}{0}{figure=plots/l4z_search2.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1900}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>You may refine your search by going back\\
                       \>to search form.
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Input form
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Bibliography input form
  \end{center}}
}
%%
%%  Show message form window
%%
\putbox{p}{ct}{c}{c}{350}{1800}{0}{figure=plots/l4z_input.eps,clip=}
%%
%%  Some explanations
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{ct}{c}{c}{1800}{s}{0}{%
  \vspace*{5.mm}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Mechanism to avoid duplicate identifiers\\[2.mm]
  \ \cbull{\red}{-.5em}\>Mechanism to modify exsting entries\\
                       \>(have to be checked by editor)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Detailed online help\\[2.mm]
  \ \cbull{\red}{-.5em}\>Please adhere to format conventions!
  \end{tabbing}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Life Cycle of a \LaTeXZ BiBTeX entry
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{250}{%
  \begin{center}
  \large\bf Life Cycle of a \LaTeXZ\\[-3.mm]
            BiBTeX entry
  \end{center}}
}
%%
%%  stations
%%
{
\SetWidth{12.0}
\SetColor{Red}
\ArrowLine(450,2150)(450,1650)
\ArrowLine(450,1600)(450,1000)
\ArrowLine(450,1050)(450,350)
}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{350}{900}{0}{%
  \begin{center}
  Entry by user\\
  {\small\darkblue (can be used, preliminary)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{850}{900}{0}{%
  \begin{center}
  Entry into\\
  \LaTeXZ data base\\
  {\small\darkblue (fully autorized usage)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{1450}{900}{0}{%
  \begin{center}
  Update by user\\
  {\small\darkblue (main entry unchanged, update can be used)}
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkgreen}{lightpink}{darkgreen}
\putbox{f}{lt}{c}{0}{2050}{900}{0}{%
  \begin{center}
  Update in data base\\
  {\small\darkblue (main entry changed, 
  old and temporary versions may remain
  available if necessary)}
  \end{center}
}}
%%
%%  actions
%%
{
\SetWidth{12.0}
\SetColor{Red}
\LongArrow(1000,1900)(500,1900)
\LongArrow(1000,1300)(500,1300)
\LongArrow(1000,700)(500,700)
}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{720}{750}{0}{%
  \begin{center}
  Check by scientific editor\\
  {\small\darkred 
   (reference data,\\ 
   identifier,\\
   \LaTeX\ formatting)

  }
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{1320}{750}{0}{%
  \begin{center}
  Mistake, change,\\
  missing information\\
  detected by user\\
  {\small\darkred 
   (use update mode\\ 
   of \LaTeXZ\\
   input form)

  }
  \end{center}
}}
{\putboxparloc{}{1.pt}{darkblue}{lightyellow}{black}
\putbox{f}{rc}{c}{-0}{1920}{750}{0}{%
  \begin{center}
  Check by scientific editor\\
  {\small\darkred 
   (keep old identifiers\\ 
   connected to\\
   updated data)

  }
  \end{center}
}}
%%
\end{boxpage}
%-------------------------------------------------------------------------------
%       Status and Release
%-------------------------------------------------------------------------------
\begin{boxpage}
%%
%%  header box
%%
{\putboxparloc{}{1.pt}{darkblue}{yellow}{darkblue}
\putbox{f}{ct}{c}{c}{0}{s}{200}{%
  \begin{center}
  \large\bf Status and Release
  \end{center}}
}
%%
%%  Status
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{lt}{c}{0}{300}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Status:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>First tests successful\\[-2.mm]
                       \>(thanks to Brian Foster, Alex Kappes,\\[-2.mm]
                       \>Matthew Wing for giving it a try)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Meanwhile: lots of improvements\\[-2.mm]
                       \>implemented\\[2.mm]
  \ \cbull{\red}{-.5em}\>Some details have to be finalized.
  \end{tabbing}
}}
%%
%%  Your response
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{lt}{c}{0}{1700}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Your response:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>{\red Give it a try!}\\[2.mm]
  \ \cbull{\red}{-.5em}\>{\red Please} report problems, criticism,\\[-2.mm]
                       \>suggestions, comments\\[-2.mm]
                       \>(use the message form!)\\[2.mm]
  \ \cbull{\red}{-.5em}\>It is like investing some work now\\[-2.mm]
                       \>to save much more work later\dots
  \end{tabbing}
}}
%%
%%  Release
%%
{\putboxparloc{}{2.pt}{darkgreen}{lightyellow}{darkblue}
\putbox{f}{rt}{c}{-0}{1070}{1400}{0}{%
  \vspace*{-12.mm}
  \begin{center}{\large\magenta Release:}\end{center}
  \begin{tabbing}
  dd\ \cbull{\red}{-.5em}\=\ \cmin{\red}{.5em}\=\kill
  \ \cbull{\red}{-.5em}\>Expected in the next days\\[-2.mm]
                       \>(not later than end of next week)\\[2.mm]
  \ \cbull{\red}{-.5em}\>Will be announced to zeus+all\\[2.mm]
  \ \cbull{\red}{-.5em}\>It's already usable, though! 
  \end{tabbing}
}}
%%
\end{boxpage}


==> LaTeX/user/predef.tex <==
% all predefined commands are below:
% for table, figure, references:
\def\Fref#1{Figure~\ref{#1}}                    % ref to figures 
\def\fref#1{figure~\ref{#1}}
\def\Tref#1{Table~\ref{#1}}                     % ref to tables
\def\tref#1{table~\ref{#1}}
\def\Cref#1{Chapter~\ref{#1}}                   % ref to chapters
\def\cref#1{chapter~\ref{#1}}
\def\Sref#1{Section~\ref{#1}}                   % ref to sections
\def\sref#1{section~\ref{#1}}
% equations:
%\newcommand{\beqn}{\begin{eqnarray}}
%\newcommand{\eeqn}{\end{eqnarray}}
\def\Eref#1{Equation~\ref{#1}}
\def\eref#1{equation~\ref{#1}}

% for D star:
% \newcommand{\fcharm}{\mbox{$F_2^{charm}$}}
\newcommand{\fcharm}{\mbox{$F_2^{c\overline{c}}$}}
\newcommand{\dstar}{\mbox{$D^\star$}}
\newcommand{\dzero}{\mbox{$D^0$}}
\newcommand{\pislow}{\mbox{$\pi_{slow}$}}
\newcommand{\pis}{\mbox{$\pi_{slow}$}}
\newcommand{\pislowq}{\mbox{$\pi_{slow}^{+}$}}
\newcommand{\kpipi}{\mbox{$K\pi\ \pislow $}}
\newcommand{\kpipiq}{\mbox{$K^{-}\pi^{+} \pislowq $}}
\newcommand{\kthreepi}{\mbox{$K3\pi\ \pislow $}}
\newcommand{\kthreepiq}{\mbox{$K^{-} \pi^{-} \pi^{+} \pi^{+} \pislowq $}}
\newcommand{\etadstar}{\mbox{$|\eta (\dstar)|$}}
\newcommand{\dm}{\mbox{$\Delta M$}}
\newcommand{\deltam}{\mbox{$\Delta M$}}
\newcommand{\mdz}{\mbox{$M(\dzero)$}}
\newcommand{\ccbar}{\mbox{$c\overline{c}$}}

% other 
\newcommand{\jpsi}{\mbox{$J/ \psi$}}    % J/psi

% kinematical variables:
\newcommand{\yel}{\mbox{$y_{el}$}}
\newcommand{\yjb}{\mbox{$y_{JB}$}}
\newcommand{\qtwo}{\mbox{$Q^2$}}
\newcommand{\PT}{\mbox{$P_{T}$}}
\newcommand{\zvtx}{\mbox{$|z_{vtx}|$}}
\newcommand{\eminpz}{\mbox{$E-p_{z}$}}
\newcommand{\mx}{\mbox{$M_{x}$}}
\newcommand{\cmx}{\mbox{$C_{M_{x}}$}}
\newcommand{\mxmeas}{\mbox{$M_{x}^{MEAS}$}}
\newcommand{\mxtrue}{\mbox{$M_{x}^{TRUE}$}}
\newcommand{\gamp}{\mbox{$\gamma^{*} p$}}
\newcommand{\lint}{\mbox{$\cal{L}$$_{int}$}}
\newcommand{\msbar}{\mbox{$\overline{MS}$}}

% diffractive:
\newcommand{\etamax}{\mbox{$\eta_{max}$}}
\newcommand{\etamaxtru}{\mbox{$\eta_{max}^{TRUE}$}}
\newcommand{\etamaxrec}{\mbox{$\eta_{max}^{REC}$}}
\newcommand{\pom}  {I\hspace{-0.27em}P}
\newcommand{\xpom} {\mbox{$x_{_{\pom}}$}}
\newcommand{\xpomeron} {\mbox{$\xpom$}}











==> LaTeX/user/predeffonts.tex <==
% Put predefined fonts here:

\font\sansbig   = phvr  at 26pt
\font\sansbigb  = phvbo at 11pt  %scaled 1700
\font\sansbb    = phvb  at 12pt  %scaled 1700
\font\sans      = phvb  at 11pt  %scaled 1700
\font\sansi     = phvbo at 10pt  %scaled 1700
\font\sansii    = phvbo at 9pt   %scaled 1700
%\font\sans     = phvr  at 22pt  %scaled 1700
\font\sansb     = phvb  at 22pt  %scaled 1700
\font\sansbi    = phvbo at 22pt  %scaled 1700
\font\sanss     = phvr  at 19pt  %scaled 1700
\font\sanssb    = phvb  at 19pt  %scaled 1700
\font\sanssbi   = phvbo at 19pt  %scaled 1700
\font\sanssi    = phvro at 10pt  %scaled 1700
\font\sanssii   = phvro at 9pt   %scaled 1700
\font\sansvs    = phvr  at 17pt  %scaled 1700
\font\sansvsi   = phvro at 17pt  %scaled 1700
\font\sanssiii  = phvro at 7pt   %scaled 1700
\font\sanssiib  = phvbo at 7pt   %scaled 1700

%Helvetica Regular
\font\helva	= phvr  at 7pt  
\font\helvb	= phvr  at 8pt
\font\helvc	= phvr  at 9pt
\font\helvd	= phvr  at 10pt
\font\helve	= phvr  at 11pt
\font\helvf	= phvr  at 12pt
\font\helvg	= phvr  at 13pt
\font\helvh	= phvr  at 14pt
\font\helvi	= phvr  at 15pt
\font\helvj	= phvr  at 16pt
\font\helvk	= phvr  at 17pt
\font\helvl	= phvr  at 18pt
\font\helvm	= phvr  at 19pt
\font\helvn	= phvr  at 20pt
\font\helvo	= phvr  at 21pt
\font\helvp	= phvr  at 22pt
\font\helvq	= phvr  at 23pt
\font\helvr	= phvr  at 24pt
\font\helvs	= phvr  at 25pt
\font\helvt	= phvr  at 26pt
\font\helvu	= phvr  at 27pt
\font\helvv	= phvr  at 28pt
\font\helvw	= phvr  at 29pt
\font\helvx	= phvr  at 30pt

%Helvetica Italics
\font\helvia	= phvro  at 7pt  
\font\helvib	= phvro  at 8pt
\font\helvic	= phvro  at 9pt
\font\helvid	= phvro  at 10pt
\font\helvie	= phvro  at 11pt
\font\helvif	= phvro  at 12pt
\font\helvig	= phvro  at 13pt
\font\helvih	= phvro  at 14pt
\font\helvii	= phvro  at 15pt
\font\helvij	= phvro  at 16pt
\font\helvik	= phvro  at 17pt
\font\helvil	= phvro  at 18pt
\font\helvim	= phvro  at 19pt
\font\helvin	= phvro  at 20pt
\font\helvio	= phvro  at 21pt
\font\helvip	= phvro  at 22pt
\font\helviq	= phvro  at 23pt
\font\helvir	= phvro  at 24pt
\font\helvis	= phvro  at 25pt
\font\helvit	= phvro  at 26pt
\font\helviu	= phvro  at 27pt
\font\helviv	= phvro  at 28pt
\font\helviw	= phvro  at 29pt
\font\helvix	= phvro  at 30pt

%Helvetica Bold
\font\helvba	= phvb  at 7pt  
\font\helvbb	= phvb  at 8pt
\font\helvbc	= phvb  at 9pt
\font\helvbd	= phvb  at 10pt
\font\helvbe	= phvb  at 11pt
\font\helvbf	= phvb  at 12pt
\font\helvbg	= phvb  at 13pt
\font\helvbh	= phvb  at 14pt
\font\helvbi	= phvb  at 15pt
\font\helvbj	= phvb  at 16pt
\font\helvbk	= phvb  at 17pt
\font\helvbl	= phvb  at 18pt
\font\helvbm	= phvb  at 19pt
\font\helvbn	= phvb  at 20pt
\font\helvbo	= phvb  at 21pt
\font\helvbp	= phvb  at 22pt
\font\helvbq	= phvb  at 23pt
\font\helvbr	= phvb  at 24pt
\font\helvbs	= phvb  at 25pt
\font\helvbt	= phvb  at 26pt
\font\helvbu	= phvb  at 27pt
\font\helvbv	= phvb  at 28pt
\font\helvbw	= phvb  at 29pt
\font\helvbx	= phvb  at 30pt

%Helvetica Bold Italic
\font\helvbia	= phvbo  at 7pt  
\font\helvbib	= phvbo  at 8pt
\font\helvbic	= phvbo  at 9pt
\font\helvbid	= phvbo  at 10pt
\font\helvbie	= phvbo  at 11pt
\font\helvbif	= phvbo  at 12pt
\font\helvbig	= phvbo  at 13pt
\font\helvbih	= phvbo  at 14pt
\font\helvbii	= phvbo  at 15pt
\font\helvbij	= phvbo  at 16pt
\font\helvbik	= phvbo  at 17pt
\font\helvbil	= phvbo  at 18pt
\font\helvbim	= phvbo  at 19pt
\font\helvbin	= phvbo  at 20pt
\font\helvbio	= phvbo  at 21pt
\font\helvbip	= phvbo  at 22pt
\font\helvbiq	= phvbo  at 23pt
\font\helvbir	= phvbo  at 24pt
\font\helvbis	= phvbo  at 25pt
\font\helvbit	= phvbo  at 26pt
\font\helvbiu	= phvbo  at 27pt
\font\helvbiv	= phvbo  at 28pt
\font\helvbiw	= phvbo  at 29pt
\font\helvbix	= phvbo  at 30pt






==> LaTeX/zeus/zeus_other_def.tex <==
%------------------------------------------------------------------------------
%       Standard ZEUS text fragments
%       ----------------------------
%       -> references system footnote
%------------------------------------------------------------------------------
\newcommand{\ZcoosysA}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the center of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\ZcoosysB}{%
The ZEUS coordinate system is a right-handed Cartesian system, with the $Z$
axis pointing in the proton beam direction, referred to as the ``forward
direction'', and the $X$ axis pointing left towards the centre of HERA.
The coordinate origin is at the nominal interaction point.\xspace}
\newcommand{\Zpsrap}{%
The pseudorapidity is defined as $\eta=-\ln\left(\tan\frac{\theta}{2}\right)$,
where the polar angle, $\theta$, is measured with respect to the proton beam
direction.\xspace}
\newcommand{\ZcoosysfnA}{\footnote{\ZcoosysA}}
\newcommand{\ZcoosysfnB}{\footnote{\ZcoosysB}}
\newcommand{\ZcoosysfnAeta}{\footnote{\ZcoosysA\Zpsrap}}
\newcommand{\ZcoosysfnBeta}{\footnote{\ZcoosysB\Zpsrap}}
%------------------------------------------------------------------------------
%       -> introductory sentence for detector description
%------------------------------------------------------------------------------
\newcommand{\Zdetdesc}{%
A detailed description of the ZEUS detector can be found 
elsewhere~\cite{zeus:1993:bluebook}. A brief outline of the 
components that are most relevant for this analysis is given
below.\xspace}
%------------------------------------------------------------------------------
%       -> CTD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctddesc}[1]{%
Charged particles were tracked in the central tracking detector (CTD)~\citeCTD,
which operated in a magnetic field of $1.43\Tesla$ provided by a thin 
superconducting coil. The CTD consisted of 72~cylindrical drift chamber 
layers, organized in 9~superlayers covering the polar-angle#1 region 
\mbox{$15^\circ<\theta<164^\circ$}. The transverse-momentum resolution for
full-length tracks is $\sigma(p_T)/p_T=0.0058p_T\oplus0.0065\oplus0.0014/p_T$,
with $p_T$ in $\Gev$.}
%------------------------------------------------------------------------------
%       -> CTD/MVD description (coordinate system footnote is given as argument)
%------------------------------------------------------------------------------
\newcommand{\Zctdmvddesc}[1]{%
In the kinematic range of the analysis, charged particles were tracked
in the central tracking detector (CTD)~\citeCTD, and the microvertex
detector (MVD)~\citeMVD,. These components operated in a magnetic
field of $1.43\Tesla$ provided by a thin superconducting solenoid. The
CTD consisted of 72~cylindrical drift chamber layers, organised in
nine superlayers covering the polar-angle#1 region
\mbox{$15^\circ<\theta<164^\circ$}. The MVD consisted of a barrel
(BMVD) and a forward (FMVD) section with three cylindrical layers and
four vertical planes of single-sided silicon strip sensors in the BMVD
and FMVD respectively. The BMVD provided polar-angle coverage for
tracks with three measurements from $30^\circ$ to $150^\circ$. The
FMVD extended the polar-angle coverage in the forward region to
$7^\circ$. After alignment the single hit resolution of the BMVD was
$\rm 25\,\mu m$ and the impact parameter resolution of the CTD-BMVD system
for high momentum tracks was $\rm 100\,\mu m$.}
%------------------------------------------------------------------------------
%       -> CAL description
%------------------------------------------------------------------------------
\newcommand{\Zcaldesc}{%
The high-resolution uranium--scintillator calorimeter (CAL)~\citeCAL consisted 
of three parts: the forward (FCAL), the barrel (BCAL) and the rear (RCAL)
calorimeters. Each part was subdivided transversely into towers and
longitudinally into one electromagnetic section (EMC) and either one (in RCAL)
or two (in BCAL and FCAL) hadronic sections (HAC). The smallest subdivision of
the calorimeter is called a cell.  The CAL energy resolutions, as measured under
test-beam conditions, are $\sigma(E)/E=0.18/\sqrt{E}$ for electrons and
$\sigma(E)/E=0.35/\sqrt{E}$ for hadrons ($E$ in $\Gev$).}
%------------------------------------------------------------------------------
%       -> MUON description
%------------------------------------------------------------------------------
\newcommand{\Zmuondesc}{%
The muon system consisted of rear, barrel (R/BMUON) and forward
(FMUON) tracking detectors. The B/RMUON consisted of limited--streamer
(LS) tube chambers placed behind the BCAL (RCAL), inside and outside a
magnetized iron yoke surrounding the CAL. The barrel and rear muon
chambers cover polar angles from $34^\circ$ to $135^\circ$ and from
$135^\circ$ to $171^\circ$, respectively. The FMUON consisted of six
trigger planes of LS tubes and four planes of drift chambers covering
the angular region from $5^\circ$ to $32^\circ$. The muon system
exploited the magnetic field of the iron yoke and, in the forward
direction, of two iron toroids magnetized to $\approx\,1.6\,{\rm T}$
to provide an independent measurement of the muon momentum.}
%------------------------------------------------------------------------------
%       -> BAC description
%------------------------------------------------------------------------------
\newcommand{\Zbacdesc}{%
The iron yoke surrounding the CAL was instrumented with proportional
drift chambers to form the Backing Calorimeter (BAC)~\citeBAC.  The
BAC consisted of 5142 aluminium chambers inserted into the gaps
between $7.3\,cm$ thick iron plates (10, 9 and 7 layers in forecap,
barrel and rearcap, respectively) serving as calorimeter absorber.
The chambers were typically $5\,m$ long and had a wire spacing of
$1.5\,cm$. The anode wires were covered by $50\,cm$ long cathode
pads. The BAC was equipped with energy
readout and position sensitive readout for muon tracking.  The former
was based on 1692 pad towers ($50 \times 50\,cm^2$), providing an
energy resolution of $\sim 100\%/\sqrt E$. The position information
from the wires allowed the reconstruction of muon trajectories in two
dimensions ($XY$ in barrel and $YZ$ in endcaps) with spatial accuracy
of a few $mm$.}
%------------------------------------------------------------------------------
%       -> LUMI description (The actual lumi uncertainty in percent is given as the argument) 
%------------------------------------------------------------------------------
\newcommand{\Zlumidesc}[1]{%
The luminosity was measured using the Bethe-Heitler reaction
$ep\,\rightarrow\, e\gamma p$ by a luminosity detector which consisted
of independent lead-scintillator calorimeter\citePCAL and a magnetic
spectrometer\citeSPECTRO systems. The fractional systematic
uncertainty on the measured luminosity was #1\%.}
%------------------------------------------------------------------------------
%       Handy macros, mainly for text mode:
%       -----------------------------------
%       -> unknown marker
%------------------------------------------------------------------------------
\newcommand{\xxx}{\hbox{$\qsm\qsm\qsm$}\xspace}
%------------------------------------------------------------------------------
%       -> D0 acronym
%------------------------------------------------------------------------------
\newcommand{\DO}{{D{\O}}\xspace}
%------------------------------------------------------------------------------
%       -> (anti-)something with correct hyphenation
%------------------------------------------------------------------------------
\newcommand{\Anti}[1]{\hbox{(anti-)}\discretionary{}{}{}#1}
\newcommand{\anti}[1]{(anti\discretionary{-)}{}{)}#1}
%------------------------------------------------------------------------------
%       -> characters for typewriter font (used for http addresses)
%------------------------------------------------------------------------------
\chardef\usc=95
\chardef\til=126
%------------------------------------------------------------------------------
%       -> xdotspace (like xspace, but adds period unless
%          another period follows)
%       -> "nn% C.L."
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\DeclareRobustCommand\xdotspace{\futurelet\@let@token\@xdotspace}
\def\@xdotspace{%
  \ifx\@let@token.\else
  \ifx\@let@token\bgroup.\else
  \ifx\@let@token\egroup.\else
  \ifx\@let@token\/.\else
  \ifx\@let@token\ .\else
  \ifx\@let@token~.\else
  \ifx\@let@token!.\else
  \ifx\@let@token,.\else
  \ifx\@let@token:.\else
  \ifx\@let@token;.\else
  \ifx\@let@token?.\else
  \ifx\@let@token/.\else
  \ifx\@let@token'.\else
  \ifx\@let@token).\else
  \ifx\@let@token-.\else
  \ifx\@let@token\@xobeysp.\else
  \ifx\@let@token\space.\else
  \ifx\@let@token\@sptoken.\else
   .\space
   \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\CL}[1]{$#1\%$~C.L\xdotspace}
%------------------------------------------------------------------------------
%       -> vertical rule of width zero and variable height & depth
%------------------------------------------------------------------------------
\newcommand{\stru}[2]{%
   \relax\ifmmode\hbox{\vrule height#1 depth#2 width0pt}%
   \else\vrule height#1 depth#2 width0pt\fi}
%------------------------------------------------------------------------------
%       -> underline with resonable distance text - line
%------------------------------------------------------------------------------
\newcommand{\uline}[1]{$\underline{\hbox{#1\stru{0.pt}{.485ex}}}$}
%------------------------------------------------------------------------------
%       -> roman numbers (uppercase and lowercase)
%------------------------------------------------------------------------------
\newcommand{\Ronum}[1]{\uppercase\expandafter{\romannumeral#1}}
\newcommand{\ronum}[1]{\expandafter{\romannumeral#1}}
%------------------------------------------------------------------------------
%       -> definition for LaTeX4zeus
%------------------------------------------------------------------------------
\DeclareRobustCommand{\LaTeXZ}{%
  \LaTeX\kern-.05em4\kern-.1em
  {\raisebox{-0.2ex}{$\scriptstyle\text{ZEUS}$}}\xspace}
%------------------------------------------------------------------------------
%       -> define \coll and \etal macros used in
%          LaTeX4zeus bibliography data base
%------------------------------------------------------------------------------
\newcommand{\coll}{Coll.\xspace}
\newcommand{\etal}{{\it et al.}\xspace}
%------------------------------------------------------------------------------
%       -> shorthands for equation, figure, table, section references
%          (require standard use of labels: eq-... for equations, cha-...
%           for chapters, sec-... for (sub)sections, tab-... for tables
%           and fig-... for figures)
%------------------------------------------------------------------------------
\newcommand{\eq}[1]{(\ref{eq-#1})}
\newcommand{\eqsand}[2]{(\ref{eq-#1}) and~(\ref{eq-#2})}
\newcommand{\eqsto}[2]{(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\eqstwo}[2]{(\ref{eq-#1},\ref{eq-#2})}
\newcommand{\eqsthr}[3]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3})}
\newcommand{\eqsfou}[4]{(\ref{eq-#1},\ref{eq-#2},\ref{eq-#3},\ref{eq-#4})}
\newcommand{\Eq}[1]{Equation~(\ref{eq-#1})}
\newcommand{\Eqsto}[2]{Equations~(\ref{eq-#1})--(\ref{eq-#2})}
\newcommand{\fig}[1]{Fig.~\ref{fig-#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig-#1}}
\newcommand{\figand}[2]{Figs.~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\Figand}[2]{Figures~\ref{fig-#1} and~\ref{fig-#2}}
\newcommand{\tab}[1]{Table~\ref{tab-#1}}
\newcommand{\Tab}[1]{Table~\ref{tab-#1}}
\newcommand{\taband}[2]{Tables~\ref{tab-#1} and~\ref{tab-#2}}
\newcommand{\cha}[1]{Chap.~\ref{cha-#1}}
\newcommand{\Cha}[1]{Chapter~\ref{cha-#1}}
\newcommand{\sect}[1]{Sect.~\ref{sec-#1}}
\newcommand{\Sect}[1]{Section~\ref{sec-#1}}
\newcommand{\sectand}[2]{Sects.~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\sectto}[2]{Sects.~\ref{sec-#1} to~\ref{sec-#2}}
\newcommand{\Sectand}[2]{Sections~\ref{sec-#1} and~\ref{sec-#2}}
\newcommand{\Sectto}[2]{Sections~\ref{sec-#1} to~\ref{sec-#2}}
%------------------------------------------------------------------------------
%       -> log file message
%------------------------------------------------------------------------------
\newcommand{\LogMess}[1]{\typeout{^^J==> #1^^J}}
%------------------------------------------------------------------------------
%       Some special symbols and settings for math mode:
%       ------------------------------------------------
%       -> redefine mathbf
%------------------------------------------------------------------------------
\DeclareMathAlphabet{\mathbf}{OT1}{cmr}{bx}{sl}
%------------------------------------------------------------------------------
%       -> physics units (eV and multiples)
%------------------------------------------------------------------------------
\newcommand{\eVdist}{\kern-0.06667em}
\newcommand{\Ev}{{\text{e}\eVdist\text{V\/}}}
\newcommand{\Kev}{{\text{ke}\eVdist\text{V\/}}}
\newcommand{\Mev}{{\text{Me}\eVdist\text{V\/}}}
\newcommand{\Gev}{{\text{Ge}\eVdist\text{V\/}}}
\newcommand{\Tev}{{\text{Te}\eVdist\text{V\/}}}
\newcommand{\ev}{{\,\text{e}\eVdist\text{V\/}}}
\newcommand{\kev}{{\,\text{ke}\eVdist\text{V\/}}}
\newcommand{\mev}{{\,\text{Me}\eVdist\text{V\/}}}
\newcommand{\gev}{{\,\text{Ge}\eVdist\text{V\/}}}
\newcommand{\tev}{{\,\text{Te}\eVdist\text{V\/}}}
%------------------------------------------------------------------------------
%       -> various other units
%------------------------------------------------------------------------------
\newcommand{\mb}{\,\text{mb}}
\newcommand{\mub}{\,\upmu\text{b}}
\newcommand{\nb}{\,\text{nb}}
\newcommand{\pb}{\,\text{pb}}
\newcommand{\fb}{\,\text{fb}}
\newcommand{\mubi}{\,\upmu\text{b}^{-1}}
\newcommand{\mbi}{\,\text{mb}^{-1}}
\newcommand{\nbi}{\,\text{nb}^{-1}}
\newcommand{\pbi}{\,\text{pb}^{-1}}
\newcommand{\fbi}{\,\text{fb}^{-1}}
\newcommand{\met}{\,\text{m}}
\newcommand{\nm}{\,\text{nm}}
\newcommand{\mum}{\,\upmu\text{m}}
\newcommand{\mm}{\,\text{mm}}
\newcommand{\cm}{\,\text{cm}}
\newcommand{\km}{\,\text{km}}
\newcommand{\Amp}{\,\text{A}}
\newcommand{\nA}{\,\text{nA}}
\newcommand{\muA}{\,\upmu\text{A}}
\newcommand{\mA}{\,\text{mA}}
\newcommand{\kA}{\,\text{kA}}
\newcommand{\Hz}{\,\text{Hz}}
\newcommand{\kHz}{\,\text{kHz}}
\newcommand{\MHz}{\,\text{MHz}}
\newcommand{\GHz}{\,\text{GHz}}
\newcommand{\ppm}{\,\text{ppm}}
\newcommand{\ppb}{\,\text{ppb}}
\newcommand{\scd}{\,\text{s}}
\newcommand{\ps}{\,\text{ps}}
\newcommand{\ns}{\,\text{ns}}
\newcommand{\mus}{\,\upmu\text{s}}
\newcommand{\ms}{\,\text{ms}}
\newcommand{\rad}{\,\text{rad}}
\newcommand{\murad}{\,\upmu\text{rad}}
\newcommand{\mrad}{\,\text{mrad}}
\newcommand{\gra}{\,\text{g}}
\newcommand{\pg}{\,\text{pg}}
\newcommand{\nang}{\,\text{ng}}
\newcommand{\mug}{\,\upmu\text{g}}
\newcommand{\mg}{\,\text{mg}}
\newcommand{\kg}{\,\text{kg}}
\newcommand{\Tesla}{\,\text{T}}
\newcommand{\Kelvin}{\,\text{K}}
%------------------------------------------------------------------------------
%       -> additional operators
%------------------------------------------------------------------------------
\newcommand{\odiv}{{\operatorname*{div}}}
\newcommand{\ograd}{{\operatorname*{grad}}}
\newcommand{\orot}{{\operatorname*{rot}}}
\newcommand{\odiag}{{\operatorname*{diag}}}
\newcommand{\ocov}{{\operatorname*{cov}}}
%------------------------------------------------------------------------------
%       -> fraction with slash instead of ratio bar
%------------------------------------------------------------------------------
\newcommand{\slashfrac}[2]{%
  \raisebox{0.5ex}{\ensuremath #1}\kern-0.12em/\kern-0.08em
  \raisebox{-.8ex}{\ensuremath #2}}
%------------------------------------------------------------------------------
%       -> shorthand for "integral limits below and above"
%------------------------------------------------------------------------------
\newcommand{\intl}{\int\limits}
\newcommand{\ointl}{\oint\limits}
%------------------------------------------------------------------------------
%       -> d'Alembert operator
%------------------------------------------------------------------------------
\newcommand{\sqr}[3]{%
    {\vcenter{\hrule height.#3ex\hbox{\vrule width.#2ex height#1ex
     \kern#1ex\vrule width.#3ex}\hrule height.#2ex}}}
\newcommand{\dalem}{\mathchoice\sqr{1.3}{08}{24}\sqr{1.4}{08}{24}
                    \sqr{1.15}{07}{21}\sqr{1.0}{06}{18}\,}
%------------------------------------------------------------------------------
%       -> vectors and matrices
%------------------------------------------------------------------------------
\newcommand{\vect}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\pvect}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\bvect}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\vvect}[1]{\begin{vmatrix}#1\end{vmatrix}}
\newcommand{\Vvect}[1]{\begin{Vmatrix}#1\end{Vmatrix}}
%------------------------------------------------------------------------------
%       -> antiparticles and particles with a bar in parentheses
%------------------------------------------------------------------------------
\newcommand{\widebar}[1]{%
   \mkern1.5mu\overline{\mkern-1.5mu#1\mkern-1.mu}\mkern1.mu}
\catcode`\@=11 % @ signs are now treated as letters
\newcommand{\parenbar}{\mathpalette\p@renb@r}
\def\p@renb@r#1#2{\vbox{%
  \ifx#1\scriptscriptstyle \dimen@.7em\dimen@ii.2em\else
  \ifx#1\scriptstyle \dimen@.8em\dimen@ii.25em\else
  \dimen@1em\dimen@ii.4em\fi\fi \offinterlineskip
  \ialign{\hfill##\hfill\cr
    \vbox{\hrule width\dimen@ii}\cr
    \noalign{\vskip-.3ex}%
    \hbox to\dimen@{$\mathchar300\hfil\mathchar301$}\cr
    \noalign{\vskip-.3ex}%
    $#1#2$\cr}}}
\catcode`\@=12 % @ signs are no longer letters
\newcommand{\nuan}{\parenbar{\nu}}
\newcommand{\nunubar}{\parenbar{\nu}}
\newcommand{\ppbar}{\parenbar{p}}
\newcommand{\qqbar}{\parenbar{q}}
\newcommand{\pbar}{\widebar{p}}
\newcommand{\nbar}{\widebar{n}}
\newcommand{\qbar}{\widebar{q}}
\newcommand{\dbar}{\widebar{d}}
\newcommand{\ubar}{\widebar{u}}
\newcommand{\sbar}{\widebar{s}}
\newcommand{\cbar}{\widebar{c}}
\newcommand{\bbar}{\widebar{b}}
\newcommand{\tbar}{\widebar{t}}
\newcommand{\nubar}{\widebar{\nu}}
\newcommand{\Dbar}{\widebar{D}}
\newcommand{\ebar}{\widebar{e}}
\newcommand{\Ebar}{\widebar{e}}
\newcommand{\Hebar}{\widebar{\text{He}}}
\newcommand{\Cbar}{\widebar{\text{C}}}
\newcommand{\Abar}{\widebar{\text{A}}}
\newcommand{\Kbar}{\widebar{K}}
\newcommand{\chibar}{\widebar{\chi}}
\newcommand{\LQbar}{\widebar{\rm LQ}}
%------------------------------------------------------------------------------
%       -> small numbers
%------------------------------------------------------------------------------
\newcommand{\zero}{{\scriptscriptstyle 0}}
\newcommand{\sone}{{\scriptscriptstyle 1}}
\newcommand{\stwo}{{\scriptscriptstyle 2}}
\newcommand{\sthr}{{\scriptscriptstyle 3}}
\newcommand{\sfou}{{\scriptscriptstyle 4}}
\newcommand{\sfiv}{{\scriptscriptstyle 5}}
\newcommand{\ssix}{{\scriptscriptstyle 6}}
\newcommand{\ssev}{{\scriptscriptstyle 7}}
\newcommand{\seig}{{\scriptscriptstyle 8}}
\newcommand{\snin}{{\scriptscriptstyle 9}}
\newcommand{\sten}{{\scriptscriptstyle 10}}
\newcommand{\half}{{\scriptscriptstyle 1/2}}
%------------------------------------------------------------------------------
%       -> abbreviations for common math mode symbols
%------------------------------------------------------------------------------
\newcommand{\MSbar}{\hbox{$\overline{\rm MS}$}\xspace}
\newcommand{\UO}{{\rm U}(1)_\sY}
\newcommand{\SUT}{{\rm SU}(2)_\sL}
\newcommand{\SUTH}{{\rm SU}(3)_c}
\newcommand{\SUTUO}{{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\SUTSUTUO}{{\rm SU}(3)_c\times{\rm SU}(2)_\sL\times{\rm U}(1)_\sY}
\newcommand{\alsmu}[1]{{\alpha_s(\mu_{#1}^2)}}
\newcommand{\alsmz}{{\alpha_s(M_Z^2)}}
\newcommand{\alsqs}{{\alpha_s(Q^2)}}
\newcommand{\als}{\alpha_s}
\newcommand{\ctwb}{\cos\theta_W}
\newcommand{\ctws}{\cos^2\theta_W}
\newcommand{\diff}{{\rm d}}
\newcommand{\gh}{{\gamma_h}}
\newcommand{\lsq}[1]{{\lambda_{#1}}}
\newcommand{\lsqp}[1]{{\lambda'_{#1}}}
\newcommand{\lsqpp}[1]{{{\lambda''}_{#1}}}
\newcommand{\rnge}{\hbox{$\,\text{--}\,$}}
\newcommand{\sihat}{{\hat\sigma}}
\newcommand{\sitil}{{\tilde\sigma}}
\newcommand{\stwb}{\sin\theta_W}
\newcommand{\stwss}{\sin^4\theta_W}
\newcommand{\stws}{\sin^2\theta_W}
\newcommand{\ta}{{\theta^\ast}}
\newcommand{\tilR}{\tilde R}
\newcommand{\tilS}{\tilde S}
\newcommand{\tilU}{\tilde U}
\newcommand{\tilV}{\tilde V}
\newcommand{\tl}{{\theta_\ell}}
\newcommand{\tw}{\theta_W}
%------------------------------------------------------------------------------
%       -> roman character combinations to be used in math mode, mainly
%          sub- or superscripts
%------------------------------------------------------------------------------
\newcommand{\Born}{{\rm Born}}
\newcommand{\BR}{{\rm BR}}
\newcommand{\CC}{{\rm CC}}
\newcommand{\CI}{{\rm CI}}
\newcommand{\CJ}{{\rm CJ}}
\newcommand{\DA}{{\rm DA}}
\newcommand{\DCA}{{\rm DCA}}
\newcommand{\GRV}{{\rm GRV}}
\newcommand{\IC}{{\rm IC}}
\newcommand{\ISR}{{\rm ISR}}
\newcommand{\IP}{{\rm I$\kern-0.01667em$P}\xspace}
\newcommand{\JB}{{\rm JB}}
\newcommand{\LL}{{\rm LL}}
\newcommand{\LQ}{{\rm LQ}}
\newcommand{\LR}{{\rm LR}}
\newcommand{\MC}{{\rm MC}}
\newcommand{\NC}{{\rm NC}}
\newcommand{\NS}{{\rm NS}}
\newcommand{\QPM}{{\rm QPM}}
\newcommand{\RL}{{\rm RL}}
\newcommand{\RPv}{{{\not R}_P}}
\newcommand{\RR}{{\rm RR}}
\newcommand{\SM}{{\rm SM}}
\newcommand{\bkg}{{\rm bkg}}
\newcommand{\cut}{{\rm cut}}
\newcommand{\data}{{\rm data}}
\newcommand{\sdet}{{\rm det}}
\newcommand{\dof}{{\rm dof}}
\newcommand{\eff}{{\rm eff}}
\newcommand{\elm}{{\rm elm}}
\newcommand{\evt}{{\rm evt}}
\newcommand{\exc}{{\rm exc}}
\newcommand{\fit}{{\rm fit}}
\newcommand{\had}{{\rm had}}
\newcommand{\jet}{{\rm jet}}
\newcommand{\meas}{{\rm meas}}
\newcommand{\miss}{{\rm miss}}
\newcommand{\obs}{{\rm obs}}
\newcommand{\pnt}{{\rm pnt}}
\newcommand{\sL}{{\rm L}}
\newcommand{\sR}{{\rm R}}
\newcommand{\sS}{{\rm S}}
\newcommand{\sT}{{\rm T}}
\newcommand{\sY}{{\rm Y}}
\newcommand{\sca}{{\rm sca}}
\newcommand{\sexp}{{\rm exp}}
\newcommand{\sint}{{\rm int}}
\newcommand{\smin}{{\rm min}}
\newcommand{\smax}{{\rm max}}
\newcommand{\srad}{{\rm rad}}
\newcommand{\sthe}{{\rm the}}
\newcommand{\sys}{{\rm sys}}
\newcommand{\tot}{{\rm tot}}
\newcommand{\true}{{\rm true}}
%------------------------------------------------------------------------------
%       -> some calligraphic symbols and applications
%------------------------------------------------------------------------------
\newcommand{\Cor}{{\cal C}}
\newcommand{\F}{{\cal F}}
\newcommand{\Lumi}{{\cal L}}
\newcommand{\Prob}{{\cal P}}
\newcommand{\ord}[1]{{\cal O}(#1)}
\newcommand{\ordlr}[1]{{\cal O}\left(#1\right)}
%------------------------------------------------------------------------------
%       -> some math symbols (+,-,...) for usage as mathchar's
%------------------------------------------------------------------------------
\mathchardef\qsm=63
\mathchardef\pls=43
\mathchardef\mns=512
\mathchardef\plm=518
\mathchardef\eql=61
\mathchardef\smallleft=300
\mathchardef\smallright=301
\mathchardef\les=316
\mathchardef\gre=318
\mathchardef\leq=532
\mathchardef\grq=533
%------------------------------------------------------------------------------
%       Additional functionality for tables and figures
%       -----------------------------------------------
%       -> alignment tools for tables
%------------------------------------------------------------------------------
\newcommand{\cA}{{\phantom{0}}}
\newcommand{\cB}{{\phantom{00}}}
\newcommand{\cC}{{\phantom{000}}}
\newcommand{\cD}{{\phantom{0000}}}
\newcommand{\cAp}{{\phantom{0.}}}
\newcommand{\cM}{{\phantom{\mns}}}
\newcommand{\cP}{{\phantom{\pls}}}
%------------------------------------------------------------------------------
%       -> comments on figures (allow to add axodraw and picture items)
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newcounter{pict@width}
\newcounter{pict@height}
\newlength{\pict@scale}
\setlength{\pict@scale}{0.1mm}
\newcommand{\psfigadd}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox to #2{\hspace{-\fill}\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcounter{pict@widthfst}
\newcounter{pict@widthscd}
\newcounter{pict@widthtot}
\newcommand{\psfigaddtwo}[7]{%
\setcounter{pict@widthfst}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthscd}{1*\ratio{#2+#4+\pict@scale/2}{\pict@scale}}
\setcounter{pict@widthtot}{1*\ratio{#2+#4+#6+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\hspace{-\fill}\begin{picture}(\thepict@widthtot,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#2,height=#3,clip=}}
\put(\thepict@widthscd,0){\psfig{figure=#5,width=#6,height=#3,clip=}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#7}
\end{picture}}
}
\newcommand{\psfigror}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,\thepict@height){\psfig{figure=#1,width=#3,height=#2,clip=,angle=270}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\newcommand{\psfigrol}[4]{%
\setcounter{pict@width}{1*\ratio{#2+\pict@scale/2}{\pict@scale}}
\setcounter{pict@height}{1*\ratio{#3+\pict@scale/2}{\pict@scale}}
\setlength{\unitlength}{\pict@scale}
\hbox{\begin{picture}(\thepict@width,\thepict@height)
\put(0,0){\psfig{figure=#1,width=#3,height=#2,clip=,angle=90}}
\SetScale{0.283466457}
\SetWidth{1.763889}
{#4}
\end{picture}}
}
\catcode`\@=12 % @ signs are no longer letters
%------------------------------------------------------------------------------
%       -> narrow figures in list environment
%------------------------------------------------------------------------------
\newlength\listtextwidth
\newcommand{\shiftfloat}[1]{
  \setlength{\listtextwidth}{\textwidth}
  \addtolength{\listtextwidth}{-#1}}
%------------------------------------------------------------------------------
%       -> "none" marker
%------------------------------------------------------------------------------
\newcommand{\none}{\hbox{---}}
%------------------------------------------------------------------------------
%       -> protected commands in captions
%------------------------------------------------------------------------------
\newcommand{\pcite}[1]{{\protect\cite{#1}}}
\newcommand{\pnl}{\protect{\newline}}
%------------------------------------------------------------------------------
%       -> pseudo-footnotes for tables
%------------------------------------------------------------------------------
\catcode`\@=11 % @ signs are now treated as letters
\newlength{\@tabfninsert}
\newlength{\@tabfnwidth}
\newcommand{\tabfootnote}[2]{%
  \setlength{\@tabfninsert}{0.8em}
  \setlength{\@tabfnwidth}{\textwidth}
  \addtolength{\@tabfnwidth}{-\@tabfninsert}
  \addtolength{\@tabfnwidth}{-0.4em}
  \noindent\makebox[\@tabfninsert][r]{\footnotesize$^{#1}$\hfil}\hfill%
  \parbox[t]{\@tabfnwidth}{\footnotesize #2\hfill}}
\catcode`\@=12 % @ signs are no longer letters

